STAD: Self-Training with Ambiguous Data for Low-Resource Relation Extraction

We present a simple yet effective self-training approach, named as STAD, for low-resource relation extraction. The approach first classifies the auto-annotated instances into two groups: confident instances and uncertain instances, according to the probabilities predicted by a teacher model. In contrast to most previous studies, which mainly only use the confident instances for self-training, we make use of the uncertain instances. To this end, we propose a method to identify ambiguous but useful instances from the uncertain instances and then divide the relations into candidate-label set and negative-label set for each ambiguous instance. Next, we propose a set-negative training method on the negative-label sets for the ambiguous instances and a positive training method for the confident instances. Finally, a joint-training method is proposed to build the final relation extraction system on all data. Experimental results on two widely used datasets SemEval2010 Task-8 and Re-TACRED with low-resource settings demonstrate that this new self-training approach indeed achieves significant and consistent improvements when comparing to several competitive self-training systems. Code is publicly available at https://github.com/jjyunlp/STAD

==> 4_analysis.tex <==
\section{Discussion}
In this section, we further analyze the results of our final system \textsc{NegPartialLabel}.

\subsection{Ablation Study}
To further analysis the effect of partial labeling and negative training, we perform ablation studies in this section.

\begin{table}[htb]
    \centering
    %\setlength{\tabcolsep}{2mm}     %只控制这个表格的sep，也可以外部套begingroup
    \begin{tabular}{lr}
    \toprule
         \bf Method & {\bf F1} \\
        ~~ Ours. & 81.6  \\
        ~~~ $-$ Partial Labeling & -1.4 \\
        ~~~ $-$ Negative Training & -2.3\\
        ~~~ $-$ Both & -3.4 \\
        \bottomrule
    \end{tabular}
    \caption{An ablation study for using partial labeling and negative training solution on the test set of Re-TACRED.}
    \label{tab:ablation}
\end{table}

\paragraph{Ambiguous Relations}
TODO
Analysis the most easy-confused relations.
And give some case studies.



The results is shown in Table~\ref{tab:ablation}.
From the table we can find that:
\begin{itemize}
    \item Two components works well on two benchmarks no matter with averaged micro or macro F1 scores. This indicates that the ambiguous instances is useful and the simple two-stage based fine-tuning solution is effective to relief the noise problem in auto-annotated data.
    \item If we drop both components, the performance drops rapidly. Especially for Re-TACRED, the decline is larger than the sum of two components calculated independently.
    This indicates that the two methods proposed in this work are complementary. 【不太会写】
\end{itemize}


\subsection{Effect of Different Partial Label Size $N$}
\label{noise_friendly}
%想分析啥？
%证明我们对于ambiguous 的定义是合理的，且不易受
% 想体现出，在self-training的框架下，模糊数据是很普遍的.
\begin{figure}[htbp]
    \centering
    %\includegraphics[width=0.46\textwidth]{images/max_ambiguous_label_num_analysis.png}
    \includegraphics[width=0.46\textwidth]{images/fixed_max_ambiguous_label_num_analysis.png}
    \caption{Effect of different partial label sizes.}
    \label{fig:ambiguous_num}
\end{figure}


To analyse the effect of partial label size $N$ in sampling ambiguous instances, we conduct experiments on the development set of SemEval with $N$ from 2 to 9.
%Basically, the number of ambiguous data increases, while the partial label size increases.
%But it is meaningless when $N=10$ because it equals the number of all relation types.


The results of averaged micro F1 scores are shown in Figure~\ref{fig:ambiguous_num}.
As a comparison, the experiments of \textsc{Self-Training} and \textsc{Hard Pseudo-label} are also conducted.
It is clear that the performance of \textsc{Hard Pseudo-Label} decreases as $N$ becomes larger because it introduces more unconfident instances.
As for \textsc{NegPartialLabel}, we can find that the performance is not sensitive to $N$.
A slight advantage is achieved when $N=5$ which 
is exactly half of the total number of relations.
This indicates that our partial labeling method for sampling ambiguous instances can mostly ensure the assumption that the correct label is in the candidate set.



\subsection{The Amount of Ambiguous Data}


\begin{figure}[!htb]
    \centering
    %\includegraphics[width=0.46\textwidth]{images/ambiguous_amount_and_improve.pdf}
    \includegraphics[width=0.46\textwidth]{images/fixed_ambiguous_amount_and_improve.png}
    \caption{Correlation between amount of ambiguous data and percentage improvement for each relation.}
    \label{fig:ambiguous_num_f1}
\end{figure}
In order to figure out the relevance between the number of ambiguous instances and performance changes of each relation, we analyse the results on the test set of SemEval.
The number of ambiguous instances for each relation is calculated by a weighted sum.
For example, an ambiguous instance with a candidate set of 3 relations gives a contribution of 1/3 for each relation in candidates.

Figure~\ref{fig:ambiguous_num_f1} shows the results where the histogram means the number of ambiguous instances for relations and the line chart represents the percentage performance improvement.
We can find that the amount of ambiguous data and the improvements have a positive correlation.
This indicates that sampling ambiguous data in self-training is useful.


